Meta-Learning Dynamics Forecasting Using Task Inference

Current deep learning models for dynamics forecasting struggle with generalization. They can only forecast in a specific domain and fail when applied to systems with different parameters, external forces, or boundary conditions. We propose a model-based meta-learning method called DyAd which can generalize across heterogeneous domains by partitioning them into different tasks. DyAd has two parts: an encoder which infers the time-invariant hidden features of the task with weak supervision, and a forecaster which learns the shared dynamics of the entire domain. The encoder adapts and controls the forecaster during inference using adaptive instance normalization and adaptive padding. Theoretically, we prove that the generalization error of such procedure is related to the task relatedness in the source domain, as well as the domain differences between source and target. Experimentally, we demonstrate that our model outperforms state-of-the-art approaches on both turbulent flow and real-world ocean data forecasting tasks.

==> sections/limitation.tex <==
Learning dynamical systems is an essential task in various fields such as climate, epidemics, and medical applications. Most existing methods must be trained to predict each specific system. The proposed model can be trusted to learn dynamical systems well and generalize well over a large heterogeneous domain.  However, there are still limitations of our current model. The performance of the proposed method depends on how well the weak supervision of task labels for training the encoder. Though we show the weak supervision can be easily obtained for fluid dynamics, ideal task label may not be easily found for other systems. And our model may not be suitable for low-dimensional dynamics that are not involved with space, since AdaIN and AdaPad are designed specifically for convolutional layers. In addition, the study of turbulence is related to the study of combustion and it is possible that the methods we employ to accelerate computation and improve physical accuracy could also be used to aid weapons research.   

==> sections/main_theory.tex <==
The high-level idea of our method is to learn a good representation of the dynamics that generalizes well across a heterogeneous domain and then adapt this representation to make predictions on new tasks.  Our model achieves this by learning multiple tasks simultaneously and then adapting to new tasks with domain transfer. We show that learning tasks simultaneously as opposed to independently results in a better generalization. We also find theoretical support for training the encoder and forecaster separately.  
%We provide an analysis for this procedure.  
See Appendix \ref{app:theory} for a longer treatment with proofs.
%  However, this sacrifices the potential to share learning between tasks.  We hypothesize our model's ability to distinguish different tasks allows for improved generalization in the setting of learn

 %The high-level idea of our method is to learn a good  representation of the underlying dynamics from multiple tasks,  and then transfer this representation to a target task (domain adaptation).

%\begin{definition}[Forecasting task]
%Each forecasting task $\V{x}_{t+1}=f(\V{x}_{t},\dots )$  is to learn a conditional distribution  $\mu$ over the system states $\mu: p( \V{x}_{t+1}|\V{x}_{t},\dots)$ conditioned on the sequence of previous states where $\mu$ is a probability measure. 
%\end{definition}

Suppose we have $K$ tasks $\{c_k\}_{k=1}^K \sim \mathcal{C}$, each of which is sampled from a continuous parameter space $\cC$. Here $c_k$ are the parameters of the task, which can be inferred by the encoder.  
%Let $\mu_k$ be corresponding conditional probability measure $p(\V{x}_{t},\lots,\V{x}_1|c_k)$.  
For each task $c_k$, we have a collection of data $\hat{\mu}_{c_k}$ of size $n$, sampled from $\mu_{k}$, a shorthand for $\mu_{c_k}$. 
  %Let $\T{D}=\cup_{c \in \cC} \cD_c$  be the union of data from all tasks. % Set $n$ to be the upper bound of the sample sizes $n=\max\lbrace n_1, \cdots,n_k \rbrace $. 

% In practice, we often have some intuition of the variables that dictate the domain.  Therefore,  we have two possible scenarios for the role of $c$ in dynamical systems:
% \begin{enumerate}
%     \item $c$ fully distinguishes the task: the differences in $\T{X}_k$ can be completely explained by the differences in $c_k$
%     \item $c$ partially distinguishes the task: a more realistic scenario where we only have partial knowledge of the domain. There exist latent variables $z'$ that need to be inferred from raw data. $z = [c,z']$ together can describe the behavior of the system in a domain.   
% \end{enumerate}

%For scenario 1, we have data from $K$ tasks $\{\T{X}_1, \dots, \T{X}_K\}$. Each task, we have a corresponding probability measure $\mu_k$.  

\paragraph{\textbf{Multi-task Learning Error}}
Our model performs  multi-task representation learning  \citep{maurer2016benefit} with joint risk $\epsilon = (1/K) \sum_k \epsilon_k$, which is the average risk of each task $\epsilon_k$ defined separately.  Denote the corresponding empirical risks $\hat{\epsilon}$ and $\hat{\epsilon}_k$.
% \begin{equation}
% \epsilon(f, \mu_1,\dots, \mu_K) = \frac{1}{K}\sum_{k=1}^K \mathbb{E}_{\V{x}_k^{(i)} \sim \mu_k} \left[ l \left(f \left(\V{x}_k^{(i)} \right) \right) \right]
%     \label{eqn:multi-task}
% % \end{equation}
% and corresponding empirical risks
% \[
% \hat{\epsilon}(f, \T{X}_1,\dots, \T{X}_K) = \frac{1}{K}\sum_{k=1}^K  l (f(\T{X}_k)),\qquad\qquad \hat{\epsilon}_k(f,\T{X}_k) = l(f(\T{X}_k)).
% \]
We can bound the true risk $\epsilon$ using the empirical risk $\hat{\epsilon}$ and Rademacher complexity $R(\T{F})$ of the hypothesis class $\T{F}$. The following theorem restates the main result in  \cite{ando2005framework} with simplified notations.
% % this directly generalizes the results from Pontil et al. This can also be related to multiple source domain adaptation setting
% Define empirical Rademacher complexity for samples from all tasks as 
% \begin{align}
% \hat{R}_{\T{X}}(\T{F}) = \mathbb{E}_{\sigma} \! \left[ \sup_{f\in \T{F}}\left( \frac{1}{nK} \sum_{k=1}^K\sum_{i=1}^n \sigma_k^{(i)} l(f(\V{x}_k^{(i)})) \right) \right]
%     \label{eqn:rademacher_join}
% \end{align}
% where $\{\sigma_k^{(i)}\}$ are independent binary variables $\sigma_k^{(i)} \in \{-1, 1\}$.  The Rademacher complexity is then defined $R(\T{F}) = \bbE_{\T{X}} ( \hat{R}_{\T{X}}(\T{F}))$.

\begin{theorem}\label{thm:main-jointbound}(\cite{ando2005framework}) 
Assume the loss is bounded $l \leq 1/2$. Given $n$ samples each from $K$ different forecasting tasks $\mu_{1}, \cdots, \mu_{k}$, then with probability at least $1-\delta$, the following inequality holds for each $f \in \T{F}$ in the hypothesis class:
\begin{align*}
%\frac{1}{K} \sum_k \epsilon_k(f)
\epsilon(f)
& \leq 
%\frac{1}{K} \sum_k\hat{\epsilon}_k(f)
\hat{\epsilon}(f) 
+ 2R(\T{F}) + \sqrt{\log{(1/\delta)}/(2 nK)}
\vspace{-2mm}
\end{align*}

\end{theorem}

%We can compare the generalization error of multi-task learning versus that of learning the individual tasks.  
The following inequality compares the performance for multi-task learning to learning individual tasks.  Let $R_k(\T{F})$ be the Rademacher complexity for $\T{F}$ over $\mu_{k}$.
\begin{lemma}\label{lem:main-compare_rad}
The Rademacher complexity for multi-task learning is bounded as
\[R(\T{F}) \leq (1/K) \sum_{k=1}^K R_k(\T{F}). \]
\end{lemma}

We can now compare \autoref{thm:main-jointbound} to the bound obtained by considering each task individually.   

\begin{prop}\label{prop:looser}
Assume the loss is bounded $l \leq 1/2$, then the generalization bound given by considering each task individually is
\begin{equation}
    \epsilon(f) \leq \hat{\epsilon}(f) + 2  (1/K) \sum_{k=1}^K R_k(\T{F}) + \sqrt{\log{(1/\delta)}/(2 nK)}. \label{eqn:main-individual} 
    \vspace{-2mm}
\end{equation}

%which is strictly looser than the bound from \autoref{thm:main-jointbound}.
\end{prop}

The upper bound in Theorem \ref{thm:main-jointbound} is strictly tighter than that of Proposition \ref{prop:looser} as the first terms $\hat{\epsilon}(f)$ are equal, the second term is smaller by Lemma \ref{lem:main-compare_rad} and the third is smaller since $1/\sqrt{2nK} \leq 1/\sqrt{2n}$. This helps explain why our multitask learning forecaster has better generalization than learning each task independently.  The shared data tightens the generalization bound.  Ultimately, though a tighter upper bound suggests lower error, it does not strictly imply it.  We further verify this theory in our experiments  by comparison to baselines which learn each task independently.

% \textcolor{blue}{
% \begin{align*}
% &(\hat{\epsilon}(f) + 2 \left(  (1/K) \sum_{k=1}^K R_k(\T{F}) \right) + \sqrt{\frac{\log{1/\delta}}{2 n}}) -  (\frac{1}{K} \sum_k\hat{\epsilon}_k(f) + 2R(\T{F}) + \sqrt{\frac{\log{1/\delta}}{2 nK}})\\
% = & 2 (\left(  \frac{1}{K} \sum_{k=1}^K R_k(\T{F}) \right) - R(\T{F})) + ( \sqrt{\frac{\log{1/\delta}}{2 n}}- \sqrt{\frac{\log{1/\delta}}{2 nK}})\\
% > & 0 + 0 = 0 ?
% \end{align*}}



% \textbf{Domain Adaptation Error.}
% Since we test on $c \sim \cC$ outside the training set $\lbrace c_k \rbrace$, we incur error due to domain adaptation from the source domains $\mu_{1},\ldots,\mu_{K}$ to target domain $\mu_c$ with $\mu$ being the true distribution.  Denote the corresponding empirical distributions of $n$ samples per task by $\hat{\mu}_c$.
% %corresponding to samples of size $n$ for each task by $\hat{\mu}_S$ and $\hat{\mu}_T$.
% % The domains $\mu_c$ have largely disjoint support for different $c$, and thus have very high KL divergence.  However, for nearby $c$ and $c'$, the samples $x^{(i)}$ are close in $\cX = \mathbb{R}^{d \times l}$ w.r.t. Euclidean distance.  Thus 
% %
% For similar domains, the Wasserstein distance $W_1(\mu_c,\mu_{c'})$ is small.  The bound from    \cite{redko2017theoretical} applies well to our setting as such: 

% \begin{theorem}[\cite{redko2017theoretical},Theorem 2]
% Let $\lambda = \mathrm{min}_{f \in \T{F}} \left( \epsilon_c(f) + 1/K \sum_{k=1}^K \epsilon_{c_k}(f) \right)$. There is $N = N(\zeta,\mathrm{dim}(\cD))$ such that for $n > N$, for any hypothesis $f$, with probability at least $1-\delta$,
% \begin{align*}
% \epsilon_c(f) &\leq \frac{1}{K}\sum_{k=1}^K \epsilon_{c_k}(f) +  W_1\left(\hat{\mu}_c,\frac{1}{K} \sum_{k=1}^K\hat{\mu}_{k}\right)  
% + \sqrt{2 \log (1/\delta)} \left( \sqrt{1/n} + \sqrt{1/(nK)} \right) + \lambda.
% \end{align*}

%\end{theorem}
%\label{thm:redko}
\paragraph{\textbf{Encoder versus Forecaster Error}}
Error from \ours{} may result from either the encoder $g_\phi$ or the forecaster $f_\theta$. Using \citep{redko2017theoretical}
%see Theorem \ref{thm:redko})
, we can bound the generalization error in terms of: (1) the empirical error of the encoder, (2) the empirical forecaster error on the source domains, and (3) the Wasserstein distance $W_1$ between the source and target domains.  We use Wasserstein distance since different tasks may have disjoint support and thus infinite KL divergence, however, samples from tasks $c,c'$ close in $\cC$ may be close in $W_1(\mu_{c},\mu_{c'})$ (see Appendix Fig. \ref{vis:w_dis}). Our two-stage training scheme is motivated by this decomposition for achieving generalization. 

Our hypothesis space has the form $\lbrace x \mapsto f_\theta(x,g_\phi(x)) \rbrace$ where $\phi$ and $\theta$ are the weights of the encoder and forecaster respectively.  Let $\epsilon_{\cX}$ be the error over the entire domain $\cX$, that is, for all $c$.  Let $\epsilon_{\mathtt{enc}}(g_\phi) = \bbE_{x \sim \cX}(\mathcal{L}_1(g(x),g_\phi(x))$ be the encoder error where $g \colon \cX \to \cC$ is the ground truth.  Let $\mathcal{G} = \{ g_\phi \colon \cX \to \cC \}$ be the task encoder hypothesis space.  Denote the empirical risk of $g_\phi$ by $\hat{\epsilon}_{\mathtt{enc}}(g_\phi)$. 

\begin{prop}
Assume $c \mapsto f_\theta(\cdot,c)$ is Lipschitz continuous with Lipschitz constant $\gamma$ uniformly in $\theta$ and $l \leq 1/2$.  Let $\lambda_c = \mathrm{min}_{f \in \T{F}} ( \epsilon_c(f) + 1/K \sum_{k=1}^K \epsilon_{c_k}(f) )$.  For large $n$ and probability $\geq 1-\delta$,
\begin{equation}
\begin{split}
\epsilon_{\cX}(f_\theta(\cdot,g_\phi(\cdot))) &\leq 
    \gamma  \hat{\epsilon}_{\mathtt{enc}}(g_\phi)  +  
    \frac{1}{K}\sum_{k=1}^K \hat{\epsilon}_{c_k}(f_\theta(\cdot,c_k)) \\
    &+ \bbE_{c \sim \cC}\left[  W_1\left(\hat{\mu}_c,\frac{1}{K} \sum_{k=1}^K\hat{\mu}_{c_k}\right) + \lambda_c 
    \right] +  2\gamma R(\mathcal{G}) \\
    & + 2 R(\cF) + (\gamma + 1) \sqrt{\log(1/\delta)/(2nK)}  \\
    & + \sqrt{2 \log (1/\delta)} \left( \sqrt{1/n} + \sqrt{1/(nK)} \right).
\end{split}
\end{equation}
\label{thm:combine}
\end{prop}


% \begin{prop}
% Assume $c \mapsto \mathrm{sup}_\theta(f_\theta(\cdot,c))$ is Lipschitz continuous with Lipschitz constant $\gamma$.  Then we bound 
% \begin{equation}
%     \epsilon_{\cX}(f_\theta(\cdot,g_\phi(\cdot))) \leq \gamma \epsilon_\mathtt{enc}(g_\phi) + \bbE_{c \sim \cC}\left[ \epsilon_{c}(f_\theta(x,c)) \right]
% \end{equation}
% where the first term is the error due to the encoder incorrectly identifying the task and the second term is the error due to the prediction network alone.
% \end{prop}

Although this result does not settle either the question of end-to-end versus pre-training or encoder-forecaster versus monolithic model, it quantifies the trade-offs these choices depend on.  We empirically consider both questions in the experiments section. 

%Together, we can bound the generalization error in terms of the empirical error of the forecaster on the source domains, the Wasserstein distance between the source and target domains, and the empirical error of the encoder; See  proposition \ref{thm:combine} in Appendix.


%\ry{need to bound the prediction part}
